A Programmable Approach to Neural Network Compression

Deep neural networks (DNNs) frequently contain far more weights, represented at a higher precision, than are required for the specific task which they are trained to perform. Consequently, they can often be compressed using techniques such as weight pruning and quantization that reduce both the model size and inference time without appreciable loss in accuracy. However, finding the best compression strategy and corresponding target sparsity for a given DNN, hardware platform, and optimization objective currently requires expensive, frequently manual, trial-and-error experimentation. In this paper, we introduce a programmable system for model compression called Condensa. Users programmatically compose simple operators, in Python, to build more complex and practically interesting compression strategies. Given a strategy and user-provided objective (such as minimization of running time), Condensa uses a novel Bayesian optimization-based algorithm to automatically infer desirable sparsities. Our experiments on four real-world DNNs demonstrate memory footprint and hardware runtime throughput improvements of 188x and 2.59x, respectively, using at most ten samples per search. We have released a reference implementation of Condensa at https://github.com/NVlabs/condensa.

==> Makefile <==
TOPLEVEL   := paper.tex
TARGET     := paper.pdf
DIFF_TARGET:= diff.pdf
ZIP_TARGET := 2021_arxiv_v2.zip
TARGETS    := $(TARGET)
TARGETS    += $(DIFF_TARGET)
GREY_TARGETS:= $(TARGETS:%.pdf=%-grey.pdf)
COPY_TARGETS:= $(TARGETS:%.pdf=%-copy.pdf)
ZIP_DIR    := $(basename $(ZIP_TARGET))
MAKEFILES  := Makefile

DEPFILES   :=
DEPFILES   += $(wildcard *.sty)
DEPFILES   += $(wildcard *.cls)
DEPFILES   += $(wildcard *.bib)
DEPFILES   += $(wildcard *.bst)
DEPFILES   += $(wildcard tex/*.tex)
DEPFILES   += $(wildcard img/*.pdf)
DEPFILES   += $(wildcard img/*.png)
DEPFILES   += $(wildcard code/*.py)
DEPFILES   += $(TOPLEVEL)
DEPFILES   += $(MAKEFILES)

GARBAGE    :=
GARBAGE    += comment.cut
GARBAGE    += $(TOPLEVEL:%.tex=%.log)
GARBAGE    += $(TOPLEVEL:%.tex=%.out)
GARBAGE    += $(TOPLEVEL:%.tex=%.aux)
GARBAGE    += $(TOPLEVEL:%.tex=%.dvi)
GARBAGE    += $(TOPLEVEL:%.tex=%.cb)
GARBAGE    += $(TOPLEVEL:%.tex=%.cb2)
GARBAGE    += $(TOPLEVEL:%.tex=%.bbl)
GARBAGE    += $(TOPLEVEL:%.tex=%.blg)
GARBAGE    += $(TOPLEVEL:%.tex=%.tdo)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.in)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.lua)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.out)
GARBAGE    += $(addprefix _markdown_,$(TOPLEVEL:%.tex=%))
GARBAGE    += $(addprefix _minted-,$(TOPLEVEL:%.tex=%))
GARBAGE    += $(wildcard figures/*-eps-converted-to.pdf)

# To use custom fonts, build with xelatex instead
LATEX      := pdflatex
LATEX      += -shell-escape
#LATEX       = xelatex
LATEXDIFF  := latexdiff --exclude-textcmd="section,subsection"

.PHONY: default
default: $(TARGET) $(TARGET:%.pdf=%-copy.pdf) $(TARGET:%.pdf=%-grey.pdf)

.PHONY: all
all: $(TARGETS) $(COPY_TARGETS) $(GREY_TARGETS) $(ZIP_TARGET)

$(TARGET): $(DEPFILES)

ECHO            := echo

# empty means it works, nonempty means it doesn't work
ESCAPE_WORKS    := $(shell $(ECHO) -e)
NEWLINE_WORKS   := $(shell $(ECHO) -n)

# A Makefile function
# @param 1: color (e.g., BLUE or GREEN)
# @param 2: message to be printed in the color
color_out_noline = \
             if [ -t 1 ] && [ -z "$(ESCAPE_WORKS)" ] && \
                [ -z "$(NEWLINE_WORKS)" ]; then \
               $(ECHO) -n -e "$(BASH_$1)$2$(BASH_CLEAR)"; \
             elif [ -z "$(NEWLINE_WORKS)" ]; then \
               $(ECHO) -n "$2"; \
             else \
               $(ECHO) "$2"; \
             fi
color_out = \
             if [ -t 1 ] && [ -z "$(ESCAPE_WORKS)" ]; then \
               $(ECHO) -e "$(BASH_$1)$2$(BASH_CLEAR)"; \
             else \
               $(ECHO) "$2"; \
             fi

BASH_CLEAR    := \e[0m
BASH_BLACK    := \e[0;30m
BASH_BROWN    := \e[0;33m
BASH_GRAY     := \e[0;37m
BASH_GREY     := \e[0;37m
BASH_DARKGRAY := \e[1;30m
BASH_DARKGREY := \e[1;30m
BASH_RED      := \e[1;31m
BASH_GREEN    := \e[1;32m
BASH_YELLOW   := \e[1;33m
BASH_BLUE     := \e[1;34m
BASH_PURPLE   := \e[1;35m
BASH_CYAN     := \e[1;36m
BASH_WHITE    := \e[1;37m

# print statistics of a tex file compilation
# @param $1: name of the log file
define TEX_STATS
	echo "$1 statistics:"
	echo "    ----"
	$(call color_out_noline,BLUE,  overfull:               )
	grep "^Overfull" $1 | wc -l
	$(call color_out_noline,BLUE,  underfull:              )
	grep "^Underfull" $1 | wc -l
	echo "    ----"
	$(call color_out_noline,BLUE,  total warnings:         )
	grep -i warning $1 | wc -l
	$(call color_out_noline,BLUE,  undefined citations:    )
	grep "Warning: Citation .* undefined" $1 | wc -l
	$(call color_out_noline,BLUE,  undefined references:   )
	grep "Warning: Reference .* undefined" $1 | wc -l
	$(call color_out_noline,BLUE,  duplicate labels:       )
	grep "Warning: Label .* multiply defined" $1 | wc -l
	echo "    ----"
	if [ "$$(type -P detex)" ]; then \
		$(call color_out_noline,BLUE,  total word count:       ); \
		detex $(1:%.log=%.tex) | wc -w; \
	  echo "    ----"; \
	fi
endef

%.pdf: %.tex
	@echo "$< -> $@"
	@$(LATEX) $< </dev/null >/dev/null || (tail -n 30 $*.log && false)
	@-bibtex $*  </dev/null >/dev/null
	@$(LATEX) $< </dev/null >/dev/null
	@$(LATEX) $< </dev/null >/dev/null
	@$(call TEX_STATS,$*.log)

%-copy.pdf: %.pdf
	@echo "$< -> $@"
	@cp $< $@

%-grey.pdf: %.pdf
	@echo "$< -> $@"
	@gs \
	  -sOutputFile="$@" \
	  -sDEVICE=pdfwrite \
	  -sColorConversionStrategy=Gray \
	  -dProcessColorModel=/DeviceGray \
	  -dCompatibilityLevel=1.4 \
	  -dNOPAUSE \
	  -dBATCH \
	  -q \
	  "$<"

images/%.eps: images/%.dot
	dot $< -Tps -o $@

images/%.ps: images/%.tex
	@echo "$< -> $@"
	@(cd images && $(LATEX) $(notdir $<)) </dev/null >/dev/null \
		|| (tail -n 30 $(<:%.tex=%.log) && false)

.PHONY: diff
diff: diff.pdf

diff.tex: old.tex new.tex
	@echo "old.tex + new.tex -> $@"
	@$(LATEXDIFF) old.tex new.tex 2>/dev/null > diff.tex

new.tex: latexpand $(DEPFILES)
	@echo "bisect.tex -> new.tex"
	@./latexpand --fatal --verbose --output new.tex bisect.tex 2>/dev/null

GARBAGE    += new.tex
GARBAGE    += diff.tex
TARGETS    += diff.pdf
GARBAGE    += old.log
GARBAGE    += old.out
GARBAGE    += old.aux
GARBAGE    += old.dvi
GARBAGE    += old.cb
GARBAGE    += old.cb2
GARBAGE    += old.bbl
GARBAGE    += old.blg
GARBAGE    += old.tdo
GARBAGE    += old.markdown.in
GARBAGE    += old.markdown.lua
GARBAGE    += old.markdown.out
GARBAGE    += old.pdf
GARBAGE    += new.log
GARBAGE    += new.out
GARBAGE    += new.aux
GARBAGE    += new.dvi
GARBAGE    += new.cb
GARBAGE    += new.cb2
GARBAGE    += new.bbl
GARBAGE    += new.blg
GARBAGE    += new.tdo
GARBAGE    += new.markdown.in
GARBAGE    += new.markdown.lua
GARBAGE    += new.markdown.out
GARBAGE    += new.pdf
GARBAGE    += new.tex
GARBAGE    += diff.log
GARBAGE    += diff.out
GARBAGE    += diff.aux
GARBAGE    += diff.dvi
GARBAGE    += diff.cb
GARBAGE    += diff.cb2
GARBAGE    += diff.bbl
GARBAGE    += diff.blg
GARBAGE    += diff.tdo
GARBAGE    += diff.markdown.in
GARBAGE    += diff.markdown.lua
GARBAGE    += diff.markdown.out
GARBAGE    += diff.tex

.PHONY: clean
clean:
	rm -rf $(GARBAGE)

.PHONY: veryclean
veryclean: clean
	rm -f $(TARGETS)
	rm -f $(COPY_TARGETS)
	rm -f $(GREY_TARGETS)
	rm -rf $(ZIP_DIR)
	rm -f $(ZIP_TARGET)

.PHONY: distclean
distclean: veryclean

.PHONY: zip
zip: $(ZIP_TARGET)

$(ZIP_DIR):
	@mkdir -p $(ZIP_DIR)

# @param 1: source file
# @param 2: destination directory
define COPY_TO_PATH
	mkdir -p $(strip $2)/$(strip $(dir $1))
	cp $1 $2/$1
	
endef

$(ZIP_TARGET): $(DEPFILES) | $(ZIP_DIR)
	@echo "copying files into $(ZIP_DIR)/"
	@$(foreach f,$(DEPFILES),$(call COPY_TO_PATH,$f,$(ZIP_DIR)))
	@echo "$(ZIP_DIR)/* -> $(ZIP_TARGET)"
	@zip -r $(ZIP_TARGET) $(ZIP_DIR) >/dev/null


==> tex/background.tex <==
\section{Background}


For a given task such as image classification, assume we have trained a large {\em reference} model $\overline{\bw} = \argmin_{\bw} L(\bw)$, where $L()$ denotes a {\em loss function} (e.g., cross-entropy on a given training set), and $\bw \in \mathbb{R}^P$. {\em Model compression} refers to finding a smaller model $\Theta$ that can be applied to the same task and ideally achieves the same accuracy as $\bw$.
Model compression can be performed in various ways, and Condensa currently supports two commonly used techniques: pruning and quantization. In pruning, non-zero values from $\bw$ are eliminated or ``pruned'' to obtain $\Theta$. Pruning is usually performed using some kind of thresholding (for eg., magnitude-based) and can be unstructured (prune any non-zero value) or structured (prune only {\em blocks} of non-zeros). On the other hand, quantization retains the number of parameters in $\Theta$ but assigns parameters in $\bw$ one of K codebook values, where the codebook may be fixed or adaptive. Condensa supports low-precision approximation, which refers to assigning each parameter in $\bw$ a corresponding lower-precision representation (for example, converting from 32-bit to 16-bit floating-point) and is equivalent to quantization using a fixed codebook.

\paragraph{Accuracy Recovery using L-C Algorithm:}

While the pruned model $\Theta$ can be obtained by directly zeroing out lower-magnitude parameters from the reference model $\overline{\bw}$ (a technique referred to as {\em direct compression}), the resulting $\Theta$ is generally sub-optimal w.r.t. the loss since the latter is ignored in learning $\Theta$. Instead, we desire an {\em accuracy recovery algorithm} that obtains an {\em optimally compressed model} with locally optimal loss denoted as $\Theta^{*}$ such that ${w^{*}} \equiv \Delta(\Theta^{*})$.

In this paper, we formulate model compression as a constrained optimization problem:
%\vspace{-2pt}
\begin{equation}
\text{min}_{\bw, \bf{\Theta}} L(\bw) \hspace{5 mm} \text{s.t.} \hspace{5 mm} \bw = \Delta(\Theta)
\label{eq:opt}
%\vspace{-2pt}
\end{equation}
Here, the \emph{decompression mapping} $\Delta :\Theta \in \mathbb{R}^{Q} \rightarrow \bw \in \mathbb{R}^{P}$ maps a low-dimensional parameterization to uncompressed model weights, and the \emph{compression mapping} $\Pi(\bw) = \argmin_{\Theta} \norm{\bw - \Delta(\Theta)}^{2}$ behaves
similar to the inverse of $\Delta$.
%
%
This formulation naturally supports a number of well-known compression techniques. In particular, pruning is defined as $\bw = \Delta(\Theta) = \Theta$ where $\bw$ is real and $\Theta$ is constrained to have fewer nonzero values, and low-precision approximation defines a constraint $w_i = \theta_i$ per parameter where $w_i$ is in a higher-precision representation and $\theta_i$ is in a lower-precision one.

Eq.~\ref{eq:opt} is non-convex due to two reasons: (1) the original problem of training the reference model is already non-convex for models such as DNNs, making the objective function of Eq~\ref{eq:opt} non-convex, and (2) the decompression mapping $\Delta(\Theta)$ typically adds another layer of non-convexity caused by an underlying combinatorial problem. While a number of non-convex algorithms may be used to solve Eq~\ref{eq:opt}, we focus on the augmented Lagrangian (AL) method~\cite{wright1999numerical} implemented in the L-C algorithm~\cite{carreira2018learning} in this paper, since it is relatively efficient and easy to implement. As its name indicates, the L-C algorithm alternates between two steps: a learning (L) step which trains the uncompressed model but with a quadratic regularization term, and a compression (C) step, which finds the best compression of $\bw$ (the current uncompressed model) and corresponds to the definition of compression mapping $\Pi$. Due to space restrictions, we refer the reader to~\cite{carreira2018learning} for a more detailed description of the L-C algorithm.



==> tex/tbl-speedup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[hbt!]
		\caption{Layer-wise TensorRT runtimes and speedups for filter pruning of VGG-19 on CIFAR-10. R and C denote reference and compressed models, respectively.}
        \centering
		\begin{sc}
	  %\resizebox{\textwidth}{!}{
				%\begin{tabular}{|c|c|c|c|c|c|}
				%\begin{tabularx}{.75\textwidth}{|X|c|c|c|c|r|}
				\begin{tabularx}{.75\textwidth}{Xllccr}
					%\hline
					\toprule
					\multirow{2}{*}{LAYER} & \multicolumn{2}{c}{SHAPE}            & \multicolumn{2}{c}{TIME(ms)} & \multirow{2}{*}{SPEEDUP} \\
					%\cline{2-6}
					\cmidrule{2-5}
					& \multicolumn{1}{c}{R} & \multicolumn{1}{c}{C}                 & R         & C                 &         \\
					%\hline
					\midrule
					conv1                  & 3 x 3 x 3 x 64    & 3 x 3 x 3 x 23    & 0.07      & 0.05              & 1.4$\times$    \\
					conv2                  & 3 x 3 x 64 x 64   & 3 x 3 x 23 x 58   & 0.23      & 0.11              & 2.09$\times$   \\
					conv3                  & 3 x 3 x 64 x 128  & 3 x 3 x 58 x 126  & 0.12      & 0.17              & 0.71$\times$   \\
    				conv4                  & 3 x 3 x 128 x 128 & 3 x 3 x 126 x 127 & 0.22      & 0.23              & 0.95$\times$   \\
					conv5                  & 3 x 3 x 128 x 256 & 3 x 3 x 127 x 256 & 0.22      & 0.22              & 1$\times$       \\
					conv6                  & 3 x 3 x 256 x 256 & 3 x 3 x 256 x 255 & 0.41      & 0.41              & 1$\times$       \\
					conv7                  & 3 x 3 x 256 x 256 & 3 x 3 x 255 x 251 & 0.41      & 0.41              & 1$\times$       \\
					conv8                  & 3 x 3 x 256 x 256 & 3 x 3 x 251 x 241 & 0.41      & 0.35              & 1.17$\times$       \\
					conv9                  & 3 x 3 x 256 x 512 & 3 x 3 x 241 x 214 & 0.28      & 0.16              & 1.75$\times$   \\
					conv10                 & 3 x 3 x 512 x 512 & 3 x 3 x 214 x 71  & 0.54      & 0.03              & 18$\times$   \\
					conv11                 & 3 x 3 x 512 x 512 & 3 x 3 x 71 x 30   & 0.53      & 0.02              & 26.5$\times$  \\
					conv12                 & 3 x 3 x 512 x 512 & 3 x 3 x 30 x 38   & 0.53      & 0.01              & 53$\times$  \\
					conv13                 & 3 x 3 x 512 x 512 & 3 x 3 x 38 x 48   & 0.56      & 0.03              & 18.66$\times$     \\
					conv14                 & 3 x 3 x 512 x 512 & 3 x 3 x 48 x 38   & 0.56      & 0.02              & 28$\times$     \\
					conv15                 & 3 x 3 x 512 x 512 & 3 x 3 x 38 x 48   & 0.56      & 0.02              & 28$\times$     \\
					conv16                 & 3 x 3 x 512 x 512 & 3 x 3 x 28 x 102  & 0.56      & 0.03              & 18.66$\times$     \\
					%\hline
					\bottomrule
					%\end{tabular}
				\end{tabularx}%
				%}
			\end{sc}
\label{tab:speedup}
\end{table*}
